Client-Based Intelligence for Resource Efficient Vehicular Big Data Transfer in Future 6G Network

Vehicular big data is anticipated to become the "new oil" of the automotive industry which fuels the development of novel crowdsensing-enabled services. However, the tremendous amount of transmitted vehicular sensor data represents a massive challenge for the cellular network. A promising method for achieving relief which allows to utilize the existing network resources in a more efficient way is the utilization of intelligence on the end-edge-cloud devices. Through machine learning-based identification and exploitation of highly resource efficient data transmission opportunities, the client devices are able to participate in overall network resource optimization process. In this work, we present a novel client-based opportunistic data transmission method for delay-tolerant applications which is based on a hybrid machine learning approach: Supervised learning is applied to forecast the currently achievable data rate which serves as the metric for the reinforcement learning-based data transfer scheduling process. In addition, unsupervised learning is applied to uncover geospatially-dependent uncertainties within the prediction model. In a comprehensive real world evaluation in the public cellular networks of three German Mobile Network Operators (MNOs), we show that the average data rate can be improved by up to 223 % while simultaneously reducing the amount of occupied network resources by up to 89 %. As a side-effect of preferring more robust network conditions for the data transfer, the transmission-related power consumption is reduced by up to 73 %. The price to pay is an increased Age of Information (AoI) of the sensor data.

==> tex/packages.tex <==
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{standalone}
\usepackage[nolist ]{acronym}
\usepackage{tcolorbox}

\usepackage{pdfpages}
\usepackage{tikz}
\usetikzlibrary{positioning}
\usepackage{hyperref}
\usepackage{pdfcomment}
\usepackage{hologo}


\usepackage{xstring}
\newcommand{\includestandalonewithpath}[2][]{%
	\begingroup%
	\StrCount{#2}{/}[\matches]%
	\StrBefore[\matches]{#2}{/}[\datapath]%
	\includestandalone[#1]{#2}%
	\endgroup%
}


\usepackage[utf8]{inputenc}
\usepackage{marvosym}


\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{tikz}

%\usetikzlibrary{decorations.pathreplacing,decorations.markings,positioning}
%\tikzset{radiation/.style={{decorate,decoration={expanding waves,angle=90,segment length=4pt}}}}
%\tikzset{antenna/.pic={
	%code={
		%\draw (0,0) circle (0.1cm);
		%\draw[radiation,decoration={angle=60}] (0.1cm,0) -- +(0:0.5);
	%}%
%}}

%%%%% Settings and additional Options %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%	Options and definitions for the Listing packet
%
\usepackage{listings}
\definecolor{ListingBackground}{rgb}{0.97,0.97,0.97}
%
\lstloadlanguages{C++,C,XML}	% Load the different languages that are used
\lstset{%
	aboveskip=0.5cm,			% Additional skip above a listing
	frame=lines,				% use top and bottom lines to separate the listing from the surrounding text
	numbers=left,            	% line numbers are put on the left side
	float=htbp,					% LaTeX float placement
	stepnumber=1,            	% every line gets numbered
	numbersep=4pt,           	% space between numbers and code
	numberstyle=\ttfamily\scriptsize,	% size of the line numbers
	keywordstyle=\bfseries,		% keyword style
	commentstyle=\itshape, 		% comment style
	columns=flexible, 			% flexible columns
	breaklines=true,         	% break lines if necessary
	breakatwhitespace=false,	% sets if automatic breaks should only happen at whitespace
	breakautoindent=true,    	% indent lines after a line break occured
	postbreak=\space,        	% break at spaces
	tabsize=4,               	% tab size 
	basicstyle=\ttfamily\scriptsize,	% non-proportional footnote-sized font for source code
	showspaces=false,           % show spaces adding particular underscores
	showstringspaces=false,     % underline spaces within strings
	showtabs=false,             % show tabs within strings adding particular underscores
	extendedchars=true,      	% show all signs from the Latin1 code page
	captionpos=tb,				% position of the caption (b = below, t = top)
	escapeinside={(*@}{@*)},	% escape characters to reference line numbers
	backgroundcolor=\color{ListingBackground} % set the background color for the listing
}

\usepackage{pgfplots}
\pgfplotsset{compat=newest}
\pgfplotsset{
    box plot/.style={
        /pgfplots/.cd,
%        black,				% Überschreibt alles in Schwarz
        fill=blue!30,
        only marks,
        mark=-,
        mark size=0.2em,
        /pgfplots/error bars/.cd,
        y dir=plus,
        y explicit,
    },
    box plot box/.style={
        /pgfplots/error bars/draw error bar/.code 2 args={%
            \draw  ##1 -- ++(.2em,0pt) |- ##2 -- ++(-.2em,0pt) |- ##1 -- cycle;
        },
        /pgfplots/table/.cd,
        y index=2,
        y error expr={\thisrowno{3}-\thisrowno{2}},
        /pgfplots/box plot
    },
    box plot top whisker/.style={
        /pgfplots/error bars/draw error bar/.code 2 args={%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark}%
            {\pgfplotserrorbarsmark}%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark options}%
            {\pgfplotserrorbarsmarkopts}%
            \path ##1 -- ##2;
        },
        /pgfplots/table/.cd,
        y index=4,
        y error expr={\thisrowno{2}-\thisrowno{4}},
        /pgfplots/box plot
    },
    box plot bottom whisker/.style={
        /pgfplots/error bars/draw error bar/.code 2 args={%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark}%
            {\pgfplotserrorbarsmark}%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark options}%
            {\pgfplotserrorbarsmarkopts}%
            \path ##1 -- ##2;
        },
        /pgfplots/table/.cd,
        y index=5,
        y error expr={\thisrowno{3}-\thisrowno{5}},
        /pgfplots/box plot
    },
    box plot median/.style={
        /pgfplots/box plot
    },
    boxplot/every median/.style={
    	ultra thick,dashed,cyan
    }
}

% Predefined Colors
\definecolor{flexicolor}{RGB}{46,49,146}
\definecolor{amaricolor}{RGB}{237,28,36}

\usepackage{xspace}

\usepackage[binary-units=true]{siunitx}
\sisetup{
	alsoload=binary
}

\usepackage{psfrag}
\usepackage{graphicx}
\usepackage{tabularx,booktabs}
\usepackage{multirow}
\usepackage{rotating}
%\usepackage{subfig}
\newcommand{\changefont}[3]{
\fontfamily{#1} \fontseries{#2} \fontshape{#3} \selectfont}
\renewcommand{\baselinestretch}{1}




\usepackage{multirow}

\usepackage[cmex10]{amsmath}

\usepackage[caption=false,font=footnotesize]{subfig}



\usepackage{stfloats}

\usepackage{wasysym}
\usepackage{fontawesome}
\newcommand\full{$\CIRCLE$}
\newcommand\partly{$\LEFTcircle$}
\newcommand\missing{$\Circle$}


==> tex/pkg/packages_access.tex <==
\NewSpotColorSpace{PANTONE}
\AddSpotColor{PANTONE} {PANTONE3015C} {PANTONE\SpotSpace 3015\SpotSpace C} {1 0.3 0 0.2}
\SetPageColorSpace{PANTONE}%
\captionsetup{font={bf,small,stretch=0.80},labelfont={bf,color=accessblue}}

==> tex/solution_approach.tex <==
\section{Solution Approach} \label{sec:approach}

%
% Fig. Approach
%
\dummy{Solution approach}{Solution approach}{fig:approach}
%
%
%
Fig.~\ref{fig:approach}




==> tex/tables/data_rate_prediction.tex <==
\begin{table}[ht]
	\small
	\centering
	\caption{Comparison of ....}
	\begin{tabular}{lcccc}
		\toprule
		\textbf{Study} & \textbf{Channel} & \textbf{Load} & \textbf{Mobility} & \textbf{Application} \\
		\midrule
		%
		% Samba/etal/2017a: RSRP, RSRQ, f, indoor/outdoor, Distance to cell, Speed, Average Number of Users
		%
		Samba \cite{Samba/etal/2017a} & \full & \full & \full & \missing \\
		%
		% Jomrich/etal/2018a: Signal Strength Level, Timing Advance, RSRP, RSRQ, CQI, RSSNR, average speed of vehicle
		%
		Jomrich \cite{Jomrich/etal/2018a} & \full & \partly & \full & \missing \\
		%
		% Wei/etal/2018a: RSSI, Cell Id, Lat, Lon, Orientation, Acceleration -> RNN
		%
		Wei \cite{Wei/etal/2018a} & \full & \missing & \full & \missing \\
		%
		% Cainey/etal/2014a: RSRP, RSRQ, SINR -> Linear Regression
		%
		Cainey \cite{Cainey/etal/2014a} & \full & \partly & \missing & \missing \\
		%
		% Akselrod/etal/2017a: SINR, RSSI ->
		%
		Akselrod \cite{Akselrod/etal/2017a} & \full & \missing & \missing & \missing \\
		%
		% Riihijarvi/Mahonen/2018a: C/I, RSS, Velocity -> Random Forest, ANN, Linear Regression
		%
		Riihijarvi \cite{Riihijarvi/Mahonen/2018a} & \full & \missing & \full & \missing \\
		%
		% Sliwa/Wietfeld/2019b:
		%
		Sliwa  \cite{Sliwa/Wietfeld/2019b} & \full & \partly & \full & \full \\
		\midrule
		%
		%
		%
		\textbf{This paper}  & \full & \full & \full & \full \\
		

		\bottomrule
		
	\end{tabular}
	
	\vspace{0.1cm}
	\full~Full integration, \partly~Partial integration, \missing~No integration
	
	\colorbox{red}{TODO: Consider accuracy and prediction methods?}
	
	\label{tab:data_rate_prediction}
\end{table}


